Can LLMs Act as Historians? Evaluating Historical Research Capabilities of LLMs via the Chinese Imperial Examination

While Large Language Models (LLMs) have increasingly assisted in historical tasks such as text processing, their capacity for professional-level historical reasoning remains underexplored. Existing benchmarks primarily assess basic knowledge breadth or lexical understanding, failing to capture the higher-order skills, such as evidentiary reasoning,that are central to historical research. To fill this gap, we introduce ProHist-Bench, a novel benchmark anchored in the Chinese Imperial Examination (Keju) system, a comprehensive microcosm of East Asian political, social, and intellectual history spanning over 1,300 years. Developed through deep interdisciplinary collaboration, ProHist-Bench features 400 challenging, expert-curated questions across eight dynasties, accompanied by 10,891 fine-grained evaluation rubrics. Through a rigorous evaluation of 18 LLMs, we reveal a significant proficiency gap: even state-of-the-art LLMs struggle with complex historical research questions. We hope ProHist-Bench will facilitate the development of domain-specific reasoning LLMs, advance computational historical research, and further uncover the untapped potential of LLMs. We release ProHist-Bench at https://github.com/inclusionAI/ABench/tree/main/ProHist-Bench.

==> tables/human.tex <==
\begin{tabular}{cccccc}
\toprule

&\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}LLM\\ Assistance\end{tabular}}}&\multicolumn{4}{c}{\textbf{Level}}\\
% &\multirow{2}{*}{\textbf{LLM Assistance}}&\multicolumn{4}{c}{\textbf{Level}}\\
\cmidrule{3-6}
&&\textbf{1}&\textbf{2}&\textbf{3}&\textbf{4}\\
\midrule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Untrained Human\end{tabular} }}&\XSolidBrush&10.00&10.00&10.00&10.00\\
&\Checkmark&&&&\\
\midrule
\multirow{2}{*}{\textbf{Expert}}&\XSolidBrush&&&&\\
&\Checkmark&&&&\\
\midrule
\textbf{SOTA LLM}&\Checkmark&&&&\\
\bottomrule
\end{tabular}

==> tables/llm-judge.tex <==
\begin{tabular}{c|cc|c}
\toprule

\multirow{2}{*}{\textbf{Judge Model}}&\multicolumn{2}{c|}{\textbf{Human Consisitency}}&\multirow{2}{*}{\textbf{Avg.}}\\
&\textbf{Rubric}&\textbf{Answer}&\\
\midrule
Gemini-2.5-Pro&62.00&51.00&56.50\\
GPT-4.1&47.00&68.00&57.50\\
GPT-5.2&72.00&62.00&67.00\\
Claude-3.7-Sonnet&66.00&70.00&68.00\\
GPT-5&57.00&81.00&69.00\\
Qwen3-235B-A22B&74.00&73.00&73.50\\
DeepSeek-R1&72.00&\textbf{82.00}&77.00\\
Gemini-3-Pro-Preview&\textbf{80.00}&80.00&\textbf{80.00}\\
\bottomrule
\end{tabular}

==> tables/main.tex <==
\begin{tabular}{l|cccc|ccccc}
\toprule


\multirow{2}{*}{\textbf{LLM}} & \textbf{Level-1} & \textbf{Level-2} & \textbf{Level-3} & \textbf{Level-4} & \multicolumn{5}{c}{\textbf{Overall}} \\
& \multicolumn{4}{c|}{WRS}& WRS & BLEU & METEOR & R-L & BERTScore\\          
\midrule
\multicolumn{10}{c}{\textbf{Closed-Source LLMs}} \\
\midrule
% Claude-sonnet-4.5-20250929-Thinking&&&&85.58
% GPT-5.2&11.07&77.65
% GPT-5.2-Thinking&14.08&86.45
% GPT-o3-2025-04-16&14.66&77.45
% Gemini-3-Pro-Preview&29.29&86.35
% Gemini-3-Pro-Preview-Thinking&26.73&86
% Qwen3-Max&17.71&87.08

Qwen3-235B-A22B-Thinking&&&&&&&&\\
DeepSeek-R1-0528&&&&&&&&\\
Gemini-3-Pro-Preview-Thinking&&&&&&&&\\
DeepSeek-V3.1-Terminus-Thinking&&&&&&&&\\
Gemini-2.5-Pro-Thinking&&&&&&&&\\
GPT-5-2025-08-07-Thinking&&&&&&&&\\
GPT-o3-2025-04-16&&&&&&&&\\
Qwen3-30B-A3B-Thinking&&&&&&&&\\
GPT-4.1-2025-04-14&&&&&&&&\\
\midrule
\multicolumn{10}{c}{\textbf{Open-Source LLMs}} \\
\midrule
Qwen3-235B-A22B-Thinking&&&&&&&&\\
DeepSeek-R1-0528&&&&&&&&\\
Gemini-3-Pro-Preview-Thinking&&&&&&&&\\
DeepSeek-V3.1-Terminus-Thinking&&&&&&&&\\
Gemini-2.5-Pro-Thinking&&&&&&&&\\
GPT-5-2025-08-07-Thinking&&&&&&&&\\
GPT-o3-2025-04-16&&&&&&&&\\
Qwen3-30B-A3B-Thinking&&&&&&&&\\
GPT-4.1-2025-04-14&&&&&&&&\\

\bottomrule
\end{tabular}

==> tables/metric.tex <==
\begin{tabular}{cccc}
\toprule

\multirow{2}{*}{\textbf{Metrics}}&\multicolumn{2}{c}{\textbf{Human Consisitency}}&\multirow{2}{*}{\textbf{Avg.}}\\
&\textbf{Rubric}&\textbf{Answer}&\\
\midrule
BLEU&64.64&80.23&72.44\\
ROUGE-L&67.52&80.60&74.06\\
METEOR&67.52&81.30&74.41\\
BERTScore&68.02&81.03&74.53\\

\bottomrule
\end{tabular}

==> tables/prompt.tex <==
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule

\multirow{2}{*}{\textbf{LLM}} &\multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Level-1\end{tabular} }}&\multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Level-2\end{tabular} }}&\multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Level-3\end{tabular} }}&\multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Level-4\end{tabular}}}\\
&\textbf{QA}&\textbf{CoT}&\textbf{RAG}&\textbf{QA}&\textbf{CoT}&\textbf{RAG}&\textbf{QA}&\textbf{CoT}&\textbf{RAG}&\textbf{QA}&\textbf{CoT}&\textbf{RAG}\\
\midrule
\multicolumn{13}{c}{\textbf{Closed-Source LLMs}} \\
\midrule
Qwen3-235B-A22B-Thinking&&&&&&&&&&&&\\
DeepSeek-R1-0528&&&&&&&&&&&&\\
Gemini-3-Pro-Preview-Thinking&&&&&&&&&&&&\\
DeepSeek-V3.1-Terminus-Thinking&&&&&&&&&&&&\\
Gemini-2.5-Pro-Thinking&&&&&&&&&&&&\\
GPT-5-2025-08-07-Thinking&&&&&&&&&&&&\\
GPT-o3-2025-04-16&&&&&&&&&&&&\\
Qwen3-30B-A3B-Thinking&&&&&&&&&&&&\\
GPT-4.1-2025-04-14&&&&&&&&&&&&\\
\midrule
\multicolumn{13}{c}{\textbf{Open-Source LLMs}} \\
\midrule
Qwen3-235B-A22B-Thinking&&&&&&&&&&&&\\
DeepSeek-R1-0528&&&&&&&&&&&&\\
Gemini-3-Pro-Preview-Thinking&&&&&&&&&&&&\\
DeepSeek-V3.1-Terminus-Thinking&&&&&&&&&&&&\\
Gemini-2.5-Pro-Thinking&&&&&&&&&&&&\\
GPT-5-2025-08-07-Thinking&&&&&&&&&&&&\\
GPT-o3-2025-04-16&&&&&&&&&&&&\\
Qwen3-30B-A3B-Thinking&&&&&&&&&&&&\\
GPT-4.1-2025-04-14&&&&&&&&&&&&\\

\bottomrule
\end{tabular}
